Nanosatellite Constellation and Ground Station Co-design for Low-Latency Critical Event Detection

Advancements in nanosatellite technology lead to more Earth-observation satellites in low-Earth orbit. We explore using nanosatellite constellations to achieve low-latency detection for time-critical events, such as forest fires, oil spills, and floods. The detection latency comprises three parts: capture, compute and transmission. Previous solutions reduce transmission latency, but we find that the bottleneck is capture latency, accounting for more than 90% of end-to-end latency. We present a measurement study on how various satellite and ground station design factors affect latency. We offer design guidance to operators on how to choose satellite orbital configurations and design an algorithm to choose ground station locations. For six use cases, our design guidance reduces end-to-end latency by 5.6 to 8.2 times compared to the existing system.

==> 8eval.tex <==
\section{Result}
\label{sec:result}
\label{sec:eval}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/eval/all_data_e2e_bar.pdf}
    \caption{
    \textbf{End-to-end latency across six use cases in different systems.}
    \SYS reduces end-to-end latency by \evalEtwoESYSoverPlanet\ compared to the existing system across all use cases.
    % End-to-end latency comparison. 
    % (with 160 satellite constellation and 125 km swath)
    }
    \label{fig:eval:e2e_latency_before_after}
\end{figure}


We evaluate \SYS to show several key results:

\begin{packedenumerate}
\item \SYS reduces end-to-end latency by \evalEtwoESYSoverPlanet\ compared to the existing deployment. 

\item \SYS reduces the capture latency by \evalCaptureSYSoverPlanet, with the number of orbital planes being the primary factor influencing the capture latency.

\item \SYS reduces the transmission latency by $4.9\times$.

\item The same constellation and ground station configuration chosen by \SYS achieves a consistent low capture and transmission latency in several use cases.
% different distributions of event locations. 


\end{packedenumerate}

\subsection{End-to-end results}

\sys provides a substantial benefit in terms of end-to-end latency, including both communication and capture latencies, and the benefit generalizes to all of the use case scenarios that we consider.


\mypara{End-to-end latency}
\autoref{fig:eval:e2e_latency_before_after} shows that \SYS reduces end-to-end
latency by \evalEtwoESYSoverPlanet\ compared to \Planet/\Planet.  
L2D2 reduces transmission latency, and even with 264 ground stations,
\Planet/\LLDD\ reduces end-to-end latency by \evalEtwoELLDDoverPlanet.
% 
\SYS's results are similarly beneficial across our use cases, demonstrating
that the technique is not tailored to a particular distribution of targets and
showing the benefit of bringing in target-distribution-specific information. 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{fig/eval/all_data_capture_vertical.pdf}
    % all_data_capture
    \caption{
    \textbf{Capture latency across six use cases in different systems.}
    \SYS reduces capture latency by \evalCaptureSYSoverPlanet\ compared to the existing system across all use cases.
    % Capture latency comparison. (with 160 satellite constellation and 125 km swath)
    }
    \label{fig:eval:capture_swath_bar_percentile}
\end{figure}



\mypara{Capture latency}
\autoref{fig:eval:capture_swath_bar_percentile} shows that \SYS reduces capture
latency by \evalCaptureSYSoverPlanet\ compared to Planet.
\Planet/\LLDD\ reduces transmission
latency, but has the same capture latency as \Planet/\Planet.








% \mypara{Event locations over month}
% % \SYS achieves a consistent low transmission latency across different distributions of event locations. 
% % 
% We use fire location data from 2021 for \SYS to select ground stations and report the transmission latency for fires that occur in 2022.
% \autoref{fig:tx:tx_latency_month} shows that \SYS achieves a low transmission latency over 12 months.
% 

% We also select two sets of ground stations based on fire location data from 2021, and location data from all use cases.
% \autoref{fig:tx:tx_latency_event_bar} shows that \SYS achieves low transmission latency for different events.
% % 
% Essentially, the selection algorithm reduces the overlap in coverage between ground stations so that a small number of ground stations can cover most of the Earth area. 
% Therefore, \SYS achieves a consistent low transmission latency.




